Simultaneous Scene Reconstruction and Whole-Body Motion Planning for Safe Operation in Dynamic Environments

Recent work has demonstrated real-time mapping and reconstruction from dense perception, while motion planning based on distance fields has been shown to achieve fast, collision-free motion synthesis with good convergence properties. However, demonstration of a fully integrated system that can safely re-plan in unknown environments, in the presence of static and dynamic obstacles, has remained an open challenge. In this work, we first study the impact that signed and unsigned distance fields have on optimisation convergence, and the resultant error cost in trajectory optimisation problems in 2D path planning, arm manipulator motion planning, and whole-body loco-manipulation planning. We further analyse the performance of three state-of-the-art approaches to generating distance fields (Voxblox, Fiesta, and GPU-Voxels) for use in real-time environment reconstruction. Finally, we use our findings to construct a practical hybrid mapping and motion planning system which uses GPU-Voxels and GPMP2 to perform receding-horizon whole-body motion planning that can smoothly avoid moving obstacles in 3D space using live sensor data. Our results are validated in simulation and on a real-world Toyota Human Support Robot (HSR).

==> bib.tex <==
Kolur et. al. \cite{Kolur2019} introduced POSH which considers graph-based trajectories and concurrently solves for solutions in multiple homotopy classes. POSH has the capability to dynamically switch between homotopies and has been demonstrated in multiple 2D environments with multiple obstacles. 

Schmitt et. al. introduced a kinodynamic manipulation plan-
ner which computes a sequence of constraint-based controllers derived from the underlying domain model. The result is that the robot can react to moving obstacles online


An accurate real-time 3D SLAM system based on a low-cost depth camera and GPU processing was proposed by Newcombe et al. (2011)
to reconstruct dense surfaces in indoor scenes. Whelan et al. 2012 extended to work in larger indoor environments. However, surface representations are unable to distinguish between free and unknown space, may require large memory particularly outdoors, and are often based on strong assumptions about the corresponding environment. OctoMap introduced as first open source implementation of a 3D occupancy mapping framework meeting the requirements outlined in the introduction is freely available.


\cite{Nageli2017}
fast receding horizon planner based on numerical optimization for
UAV realtime trajectory generation inc moving obstacles
Adopt a two layered approach: (i) a potential field to repel the robot from obstacles
and (ii) a hard constraint to stay outside a smaller enclosing
ellipsoid SΩs to enforce collision-free motion

\cite{Otte2016}
Sampling based replanning in dynamic environments but seems to be demosntrated in 2D and not real robots.

\cite{ITOMP} interleaves execution and planning for dynamic environments but doesn't use SDF for the dynamic obstacles.

\cite{GPUVoxels}, \cite{GPUVoxelsMobile} uses GPU-EDTs to evaluate the use of potential field (PF)
planners for translative motions of mobile aerial robot platforms. Planning manipulator motions is not within the scope of the work

\cite{Kaldestad2014} 
To the authors knowledge,
this is the first time that collision avoidance is demonstrated in
real-time on a real robot using parallel GPU processing. Demonstrate on a 7DoF KUKA Arm to avoid a moving arm. The virtual forces are sent to the robot impedance controller and thus result in a reactive movement of the robot. In our framework, collision avoidance behavior is incorporated on two levels:
1) on trajectory deformation level, i.e. xd(t) responds to
the virtual forces
2) on torque control level, i.e. according to (1) and (2)

Uses a restricted 2.5D environment model which is reset every time new depth sensor data is processed.
